Towards Dynamic Causal Discovery with Rare Events: A Nonparametric Conditional Independence Test

Causal phenomena associated with rare events occur across a wide range of engineering problems, such as risk-sensitive safety analysis, accident analysis and prevention, and extreme value theory. However, current methods for causal discovery are often unable to uncover causal links, between random variables in a dynamic setting, that manifest only when the variables first experience low-probability realizations. To address this issue, we introduce a novel statistical independence test on data collected from time-invariant dynamical systems in which rare but consequential events occur. In particular, we exploit the time-invariance of the underlying data to construct a superimposed dataset of the system state before rare events happen at different timesteps. We then design a conditional independence test on the reorganized data. We provide non-asymptotic sample complexity bounds for the consistency of our method, and validate its performance across various simulated and real-world datasets, including incident data collected from the Caltrans Performance Measurement System (PeMS). Code containing the datasets and experiments is publicly available.

==> Figure___Highway_Schematic.tex <==
\begin{figure*}[!htbp]
    \centering
    \includegraphics[scale=0.2]{Figures/Highway_Example_Schematic___Annotated.jpg}
    \caption{Schematic of the highway example. Here, players 1 (red), 2 (blue), 3 (green), and 4 (purple) navigate a kilometer-long stretch of highway and interact with each other while performing lane changes.
    % Lane centers are depicted with thin, dashed black lines, lane boundaries with thin, solid black lines, and the median strip with thick, solid black lines. 
    The ego player detects landmarks in the scene, which describe objects common to realistic highway scenarios, e.g., speed limit signs, exit signs, light poles, etc.
    % \dfknote{annotate: the median strip, which is ego, and a landmark} \frank{Edited. Also made font larger. Let me know what you think.}
    }
    \label{fig:Highway_Example_Schematic___Annotated}
\end{figure*}


==> Figure___RMS_Error.tex <==
% \begin{figure}[ht]
%     \centering
%     \includegraphics[scale=0.135]{Figures/Error_Plots___Quartiles___IBR_Order_2341.jpg}
%     \caption{Root-mean-square error of estimated positions vs. standard deviation of measurement noise, for player positions and landmarks.
%     % \dfknote{bigger font. units} \frank{Edited. How does it look now?}
%     }
%     \label{fig:Error_Plots___Quartiles___IBR_Order_2341}
% \end{figure}


\begin{figure}[ht]
    \centering
    \includegraphics[scale=0.12]{Figures/Error_Plots___Quartiles_poses_landmarks___IBR_Order_2341.jpg}
    \caption{Root-mean-square error of estimated vehicle (thick) and landmark (thin) positions vs. standard deviation of measurement noise, for player positions and landmarks.
    % \dfknote{bigger font. units} \frank{Edited. How does it look now?}
    }
    \label{fig:Error_Plots___Quartiles___IBR_Order_2341}
\end{figure}



==> temp.tex <==
% temp.tex
